Sublinear data structures for short Fr\'echet queries

We study metric data structures for curves in doubling spaces, such as trajectories of moving objects in Euclidean $\mathbb{R}^d$, where the distance between two curves is measured using the discrete Fr\'echet distance. We design data structures in an \emph{asymmetric} setting where the input is a curve (or a set of $n$ curves) each of complexity $m$ and the queries are with curves of complexity $k\ll m$. We show that there exist approximate data structures that are independent of the input size $N = d \cdot n \cdot m$ and we study how to maintain them dynamically if the input is given in the stream. Concretely, we study two types of data structures: (i) distance oracles, where the task is to store a compressed version of the input curve, which can be used to answer queries for the distance of a query curve to the input curve, and (ii) nearest-neighbor data structures, where the task is to preprocess a set of input curves to answer queries for the input curve closest to the query curve. In both cases we are interested in approximation. For curves embedded in Euclidean $\mathbb{R}^d$ with constant $d$, our distance oracle uses space in $\mathcal{O}((k \log(\epsilon^{-1}) \epsilon^{-d})^k)$ ($\epsilon$ is the precision parameter). The oracle performs $(1+\epsilon)$-approximate queries in time in $\mathcal{O}(k^2)$ and is deterministic. We show how to maintain this distance oracle in the stream using polylogarithmic additional memory. In the stream, we can dynamically answer distance queries to the portion of the stream seen so far in $\mathcal{O}(k^4 \log^2 m)$ time. We apply our techniques to the second problem, approximate near neighbor (ANN) data structures, and achieve an exponential improvement in the dependency on the complexity of the input curves compared to the state of the art.

==> euclideantexts.tex <==
\subsection{Grid construction}\label{sec:gridconstruction:euclidean} 

Here we construct an exponential grid based data structure for Fr\'echet curves.
The conceptual idea is the following: We start by computing an $\alpha$-approximate curve simplification $X_k=p_1,\ldots,p_k$ for $X$.
 We then construct an exponential grid (for points) around every $p_i$. Next, we consider all curves of complexity $k$ that can be built by using the points in all exponential grids. For each such curve $X'$, we precompute the distance to $X$. We store all such distances in a data structure that allows to retrieve the distance $\df(X',X)$ using the sequence of vertices of $X'$ as a key. 

Before we start with the actual construction, we note two facts. First, we observe that for all curves that are not too distant from $X_k$ with respect to the discrete Fr\'echet distance, we know that all points on the curve lie within the area that is covered by our exponential grids. This is true since in order for the discrete Fr\'echet distance to be at most some $\Delta$, every point has to be mapped to a point on $X_k$ within distance $\Delta$. So if the overall distance is not large, then each individual point is close to at least one point on $X_k$.

\begin{observation}\label{obs:aa}
Let $q=y_1,\ldots,y_k \in \Mk$ be a curve with $\df(q,X_k) \le \Delta$. Then for all $j\in [k]$, there exists an $i\in [k]$ such that $y_j$ lies within $B(x_i,\Delta)$.
\end{observation}

Second, we observe that if we move every point on a curve by at most some $\delta$, then the distance between that curve and any other curve changes by at most $\delta$, too. 

\begin{observation}\label{obs:bb}
Let $X=x_1,\ldots,x_m$ be an arbitrary curve, and let $\pi:[m]\to \mathbb{R}$ be a mapping that satisfies that 
\[
d(x_i,\pi(i)) \le \delta.
\]
Then
\[
|\df(X,Y) - \df(X',Y)| \le \delta.
\]
\end{observation}

%\begin{observation}
%Let $X=x_1,\ldots,x_n$ be an arbitrary curve, and let $X_k$ be an $\alpha$-approximate curve simplification for $X$. Let $\pi:[n]\to\mathbb{R}$ be a mapping that satisfies that
%\[
%d(x_i,\pi(i)) \le \frac{\epsilon}{\alpha} \cdot \df(X,X_k).
%\]
%Let $X'=\pi(1),\ldots,\pi(n)$ be the curve that results from moving every point $x_i$ to its image $\pi(i)$. 
%Then for any curve $Y=y_1,\ldots,y_m$, 
%\[
%|\df(X,Y) - \df(X',Y)| \le \epsilon\cdot \df(X,Y).
%\]
%\end{observation}
%\begin{proof}
%We keep the parameterizations of $X$ and $Y$ that constitute the Fr\'echet distance and upper bound the maximum distance between any two matched points on $X'$ and $Y$ for these parameterizations. This is an upper bound for the actual Fr\'echet distance.
%Now for each pair of points, the distance changes (by the triangle inequality) by at most $\frac{\epsilon}{\alpha} \cdot \df(X,X_k) \le \epsilon \cdot \df(X,Y)$, where the inequality follows since $X_k$ is an $\alpha$-approximate curve simplification.
%\end{proof}

For our data structure, we need exponential grids around points as a building block.
Exponential grids for points are known in the literature; we give a proof of the following statement in the appendix (Section~\ref{appendix:expgrid}) for completeness.

\begin{restatable}{lemma}{expgridlemma}\label{lem:expgrid}
Let $x \in \mathbb{R}^d$ be a point, $\epsilon\in(0,1)$, and $r_1, r_2\in\mathbb{R}$ with $r_1 < r_2$, and assume that $d$ is a constant.
Then there exists a set $\mathcal{G}(x)\subset\mathbb{R}^d$ of size $\mathcal{O}((\ln \frac{r_2}{r_1}) \cdot \epsilon^{-d})$ such that for every $y \in B(x,r_2) \backslash B(x,r_1)$, there is a point $z \in \mathcal{G}(x)$ with \begin{align}
||y-z|| \le \epsilon \cdot ||x-y||.\label{eq:lemma:expgrid}
\end{align}
\end{restatable}

Now we show the main result of this section.

\begin{theorem}\label{thm:gridproperties}
For a curve $X \in \Rdn$ and a precision parameter $\eps > 0$, it is possible to compute a set of curves $\mathcal{C}$ of size $\mathcal{O}(k^k\cdot (\ln \epsilon^{-1})^k \cdot \epsilon^{-dk})$ with the following property:
For any $q \in \Rdk$ that satisfies that $\eps \cdot \df(X,X_k)\le \df(q,X) \le \frac{1}{\eps} \cdot \df(X,X_k)$, it holds that
\begin{align*}
\df(q,X^\ast) \le \eps \cdot \df(q,X)
\end{align*}
where $X^\ast$ is a closest neighbor of $q$ in $\mathcal{G}$.
\end{theorem}
\begin{proof}
The set of curves is computed as follows. 
We compute an $\alpha$-approximate curve simplification $X_k=p_1,\ldots,p_k$ for some constant $\alpha$. %This also gives us $\df(X,X_k)/\alpha$ as a lower bound on the minimum distance between $X$ and any curve of complexity $k$.
%  Since $X_k$ is an $\alpha$-approximate curve simplification, 
Then we know that for any $Y \in \Rdk$, $\df(X,X_k) \le \alpha \cdot \df(X,Y)$.
In particular, since $q \in \Rdk$, 
\begin{align}\label{eq:approx-curve-simplification}
\df(X,X_k) \le \alpha \cdot \df(q,X) 
\end{align}
is true. This also implies
\begin{align}\label{eq:approx-curve-cor}
\df(q,X_k) \le \df(q,X) + \df(X,X_k) \le (1+\alpha) \cdot \df(q,X)
\end{align}
by the triangle inequality.

Next, we compute a set $\G(p_i)$ for all $i\in[k]$ by using Lemma~\ref{lem:expgrid}. We use 
\[
r_1=\frac{\epsilon}{\alpha} \cdot \df(X,X_k) \stackrel{\eqref{eq:approx-curve-simplification}}{\le} \epsilon \cdot \df(q,X)
\] and $r_2=\frac{1}{\epsilon} \df(X,X_k)$, i.e., $r_2/r_1=\alpha \cdot \epsilon^{-2}$, and a precision parameter of $\epsilon'=\epsilon/(\alpha+1)$.

Then we union all these sets together with $p_1,\ldots,p_k$ to obtain a set of points $\G$, i.e.,
\[
\G = \{p_1,\ldots,p_k\} \cup \bigcup_{i=1}^k \G(p_i).
\]
Notice that $\G$ is of size $\mathcal{O}(k\cdot (\ln \epsilon^{-1}) \cdot \epsilon^{-d})$ as long as $d$ is constant.

We obtain a set of curves $\mathcal{C}$ by constructing all curves that consist of $k$ points from $\G$. The cardinality of the resulting set of curves is $|G|^k$.

Now let $q=y_1,\ldots,y_k$ be any query curve that satisfies
\[
\eps \cdot \df(X,X_k)\le \df(q,X) \le \frac{1}{\eps} \cdot \df(X,X_k).
\]
By Observation~\ref{obs:a}, every point $y_j$ of $q$ lies in  $B(x_i,\frac{1}{\epsilon} \df(X,X_k))=B(x_i,r_2)$ for at least one $i\in[k]$. For every $j\in[k]$, we set $x(y_j)$ to an $x_i$ such that $y_j \in B(x_i,r_2)$ and such that $d(y_j,x_i)$ is minimal. Observe that this means that 
\begin{align}\label{eq:yjxyj}
||y_j-x(y_j)||\le \df(q,X_k) \stackrel{\eqref{eq:approx-curve-cor}}{\le} (1+\alpha) \cdot \df(q,X).
\end{align}
%we fix one $i$ for any $y_j$ arbitrarily and ignore if points lie in multiple balls. We denote the point $x_i$ with $y_j\in B(x_i,r_2)$ by $x(y_j)$.

So let $y_j$ be arbitrary. We map $y_j$ to a point $\pi(j)$.
If $y_j \in B(x(y_j),r_1)$, then we set $\pi(j)=x(y_j)$. Thus, 
\[
||y_j-\pi(j)|| \le r_1 \le \epsilon\cdot \df(q,X).
\]
If $y_j \in B(x(y_j),r_2)\backslash B(x(y_j),r_1)$, then we set $\pi(j)$ to a nearest neighbor of $y_j$ in $\G_i$. In this case,
\[
||y_j-\pi(j)|| \le \epsilon' \cdot d(y_j,x(y_j)) = \frac{\epsilon}{\alpha+1} \cdot d(y_j,x(y_j)) \stackrel{\eqref{eq:yjxyj}}{\le} \epsilon\cdot\df(q,X)
\]
 by Lemma~\ref{lem:expgrid}
Thus, 
\[
||y_j-\pi(j)|| \le \epsilon \cdot \df(q,X)
\]
for all $j \in [k]$. By Observation~\ref{obs:b}, this implies that $\df(q,q')\le \epsilon \cdot \df(q,X)$. 
Since $q'\in\mathcal{C}$, the closest neighbor $X^\ast$ of $q$ in $\mathcal{C}$ satisfies $\df(q,X^\ast)\le \df(q,q')$, and that implies the statement of the theorem.
\end{proof}

\begin{theorem}
Let $X \in \Rdn$, $X_k$ an $\alpha$-approximate curve simplification for $X$, $\eps > 0$ and $\mathcal{C}$ be a set of curves computed according to Theorem~\ref{thm:gridproperties} with precision parameter $\eps/2$.
Then the value $\Delta$ computed by \texttt{query}($q$,$X_k$, $\mathcal{C}$) satisfies 
\[
\df(q,X) \le \Delta \le (1+\epsilon)\cdot \df(q,X).
\]
\end{theorem}

\begin{proof}
We consider three cases.

If $\df(q,X_k) \le \frac{\eps}{2\alpha} \cdot \df(X,X_k)$ then we get by the triangle inequality that
\begin{align*}
\Delta = \df(X,X_k)+ \df(q,X_k)\le 2\df(q,X_k) + \df(q,X) 
\le& \df(q,X) + 2\frac{\eps}{2\alpha} \cdot \df(X,X_k) \\
\stackrel{\eqref{eq:approx-curve-simplification}}{\le}& (1+\eps)\cdot \df(q,X).
\end{align*}
Intuitively, $\df(X,X_k)$ dominates our distance estimation in this case, since $\df(q,X_k)$ is very small. By returning the sum of the two, we make sure that we never underestimate the true distance: The triangle inequality implies that
\[
\Delta = \df(X,X_k)+ \df(q,X_k) \ge \df(q,X) - \df(q,X_k) + \df(q,X_k) = \df(q,X).
\]

Similarly, if $\df(q,X_k) \ge \frac{2(\alpha+1)}{\eps}\cdot \df(X,X_k)$ then we observe that 
\begin{align*}
   \Delta=   \df(q,X_k) + \df(X,X_k)
\le \df(q,X) + 2\df(X,X_k) 
\le\ & \df(q,X) + 2\frac{\eps}{2(\alpha+1)}\cdot \df(q,X_k)\\
\stackrel{\eqref{eq:approx-curve-cor}}{\le}\ &
      (1+\eps) \cdot \df(q,X)
\end{align*}
and that
\[
\Delta =  \df(q,X_k) + \df(X,X_k)
\ge \df(q,X) - \df(X,X_k) + \df(X,X_k) = \df(q,X).
\]

In the remaining case, we use the guarantee from Theorem~\ref{thm:gridproperties}, which says that $\df(q,X^\ast) \le \frac{\eps}{2} \cdot \df(q,X)$. This implies by the triangle inequality that
\begin{align*}
    \Delta = \df(q,X^\ast)+\df(X^\ast,X)
    \le 2\df(q,X^\ast) + \df(q,X)
    \le (1+\eps)\cdot \df(q,X).
\end{align*}
Furthermore, we do not underestimate the distance since
\[
\Delta = \df(q,X^\ast) + \df(X^\ast,X) \ge \df(q,X) - \df(X^\ast,X) + \df(X^\ast,X) = \df(q,X),
\]
and that concludes the proof.
\end{proof}

\subsection{Result}

\begin{theorem}\label{thm:distoracle}
For any curve $X \in \Rdn$ for a constant $d\in\mathbb{N}^{\ge 1}$ and any $k \in \mathbb{N}^{\ge 1}$, it is possible to compute a data structure which uses space in $O(f_s(k,\eps))$ with $f_s(k,\eps):= k^k \cdot (\log \epsilon^{-1})^k \cdot \epsilon^{-dk}$ and which can answer approximate distance queries in  $\mathcal{O}(f_q(k,\eps))$ time, where $f_q(k,\eps):= k^2$. For any query curve $q \in \Rdk$ the data structure returns a value $d'(q)$ such that 
\[\df(q,x) \le d'(q) \le (1+\epsilon)\cdot \df(q,X).\]
The data structure can be built in time $\mathcal{O}(mk \cdot f_s(k,\epsilon))$ and space in $\mathcal{O}(mk+f_s(k,\epsilon))$.
\end{theorem}
\begin{proof}

Computing an approximate curve simplification takes time $\mathcal{O}(mdk)$; we will see this later in Theorem~\ref{thm:streamingeightapprox}. 
 Constructing the set of grid curves $\mathcal{C}$ takes time $\mathcal{O}(|\mathcal{C}|)=\mathcal{O}(f_s(k,\epsilon))$, and the Fr\'echet distance between any curve in $\mathcal{C}$ and $X$ can be computed in time and space $\mathcal{O}(mdk)$ using dynamic programming~\cite{eiter1994computing}, so we get a total precomputation time of $\mathcal{O}(mdk + |\mathcal{C}| \cdot mdk) \in \mathcal{O}(mk \cdot f_s(k,\epsilon))$ (recall that $d$ is assumed to be constant). 
We store all precomputed distances, and also $X_k$ and $\df(X,X_k)$. This requires $\mathcal{O}(|\mathcal{C}|+k)\in \mathcal{O}(f_s(k,\epsilon))$ space.  

For a query curve $q \in \Rdk$, we need to compute the Fr\'echet distance between $q$ and $X_k$, which takes time $\mathcal{O})(k^2)$, and to find the nearest neighbor $X^\ast$ of $q$ in $\mathcal{C}$. 
\todo{talk about snapping and lookup table here..}
\end{proof}

Notice that if we want to be able to answer queries for curves $q \in \XX^d_{k'}$ for all $k' \in \{1,\ldots,k\}$, we can use $k$ copies of the above data structure, which increases the storage to by only a factor of $k$ (which is small in comparison to $f_s(k,\epsilon)$).\footnote{Note that we could also use the same data structure and make the queries artificially longer by adding dummy vertices, repeating the last point of the sequence $k-k'$ times.}


==> fig-algo-example.tex <==
\tikzset{node/.style={inner sep=0cm,minimum width=0.1cm,circle, draw,fill}}
\tikzset{inxk/.style={node,minimum width=0.15cm,minimum height=0.15cm, rectangle}}
\tikzset{candidate/.style={inxk,fill=none}}

\begin{figure}
    %\centering
    \begin{subfigure}[b]{\textwidth}
%\centering
\begin{tikzpicture}[
every node/.style={node}
]

\useasboundingbox (-0.5,-1.5) rectangle (10.5,2.5);
\clip (-0.5,-1.5) rectangle (10.5,2.5);

\node (x1) at (0,0) [label=above:{$x_1$}]  {};
\node (x2) at (1,1) {};
\node (x3) at (3,2) {};
\node (x4) at (3.5,1.5) {};
\node (x5) at (5.5,1.25) {};
\node (x6) at (5.8,0.75) {};
\node (x7) at (7.3,0.9) {};
\node (x8) at (8,0) {};
\node (x9) at (8.6,-0.5) {};
\node (xn) at (10,-1) [label=above:{$x_n$}] {};

\draw [black] plot coordinates {(x1) (x2) (x3) (x4) (x5) (x6) (x7) (x8) (x9) (xn)};

\end{tikzpicture}

        \caption{A Fr\`echet curve $X=x_1,\ldots,x_n$.}
        \label{fig:algoexample:a}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{\textwidth}
%\centering        
\begin{tikzpicture}[
every node/.style={inner sep=0cm,minimum width=0.1cm,circle, draw,fill}
]

\useasboundingbox (-0.5,-1.5) rectangle (10.5,3.0);
\clip (-0.5,-1.5) rectangle (10.5,2.5);

\node (x1) at (0,0) [inxk,label=above:{$x_1$}]  {};
\node (x2) at (1,1) {};
\node (x3) at (3,2) {};
\node (x4) at (3.5,1.5) {};
\node (x5) at (5.5,1.25) [candidate] {};
\node (x6) at (5.8,0.75) {};
\node (x7) at (7.3,0.9) {};
\node (x8) at (8,0) {};
\node (x9) at (8.6,-0.5) {};
\node (xn) at (10,-1) [inxk,label=above:{$x_n$}] {};

\draw [black] plot coordinates {(x1) (x2) (x3) (x4) (x5) (x6) (x7) (x8) (x9) (xn)};

\draw [dashed] (x1) -- (x4);
\draw [dashed] (xn) -- (x5);

\draw (x1) circle (3.807);
\draw (xn) circle (5.031cm);
\end{tikzpicture}

        \caption{The vertices $x_1$ and $x_n$ form the simplification for $k=2$.}
        \label{fig:algoexample:b}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{\textwidth}
%\centering
\begin{tikzpicture}[
every node/.style=
]

\useasboundingbox (-0.5,-1.5) rectangle (10.5,3.0);
\clip (-0.5,-1.5) rectangle (10.5,2.5);

\node (x1) at (0,0) [inxk,label=above:{$x_1$}]  {};
\node (x2) at (1,1) {};
\node (x3) at (3,2) [candidate] {};
\node (x4) at (3.5,1.5) {};
\node (x5) at (5.5,1.25) [inxk] {};
\node (x6) at (5.8,0.75) {};
\node (x7) at (7.3,0.9) {};
\node (x8) at (8,0) {};
\node (x9) at (8.6,-0.5) {};
\node (xn) at (10,-1) [inxk,label=above:{$x_n$}] {};

\draw [black] plot coordinates {(x1) (x2) (x3) (x4) (x5) (x6) (x7) (x8) (x9) (xn)};

\draw (x1) circle (1.414cm);
\draw (x5) circle (2.61cm);
\draw (xn) circle (2.236cm);
%\draw [dashed] (x1) -- (x2);
\draw [dashed] (x3) -- (x5);
\draw [dashed] (x8) -- (xn);
\end{tikzpicture}

       
        \caption{The third point on the simplification has cut out an interval.}
        \label{fig:algoexample:c}
    \end{subfigure}
		    \begin{subfigure}[b]{\textwidth}
%\centering   
\begin{tikzpicture}[
every node/.style={inner sep=0cm,minimum width=0.1cm,circle, draw,fill}
]

\useasboundingbox (-0.5,-1.5) rectangle (10.5,3.0);
\clip (-0.5,-1.5) rectangle (10.5,2.5);

\node (x1) at (0,0) [inxk,label=above:{$x_1$}]  {};
\node (x2) at (1,1) {};
\node (x3) at (3,2) [inxk] {};
\node (x4) at (3.5,1.5) {};
\node (x5) at (5.5,1.25) [inxk] {};
\node (x6) at (5.8,0.75) {};
\node (x7) at (7.3,0.9) {};
\node (x8) at (8,0) [candidate] {};
\node (x9) at (8.6,-0.5) {};
\node (xn) at (10,-1) [inxk,label=above:{$x_n$}] {};

\draw [black] plot coordinates {(x1) (x2) (x3) (x4) (x5) (x6) (x7) (x8) (x9) (xn)};

\draw (x1) circle (1.414cm);
\draw (x3) circle (0.707cm);
\draw (x5) circle (1.834cm);
\draw (xn) circle (2.236cm);
\draw [dashed] (x3) -- (x4);
\draw [dashed] (x5) -- (x7);
\draw [dashed] (x8) -- (xn);
\end{tikzpicture}
				\caption{The simplification with four points.}
        \label{fig:algoexample:d}
    \end{subfigure}   
    \caption{A sample run of the approximate curve simplification algorithm.}\label{fig:algoexample}
\end{figure}


==> fig-redivision.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}
\useasboundingbox (-0.5,-1) rectangle (8.5,1);
\clip (-0.5,-0.75) rectangle (8.5,0.75);

\coordinate (pc) at (1,0);
\coordinate (pcs) at (6.5,0);
\draw [gray=black!5, fill=black!5] (pc) circle (2.7); 
\draw [gray=black!5, fill=black!5] (pcs) circle (2.7); 

\foreach \x in {0,0.5,...,8} {
\node [draw=gray,inner sep=0cm,minimum height=0.1cm] at (\x,0) {};
}

\node [draw,fill,inner sep=0cm,minimum height=0.1cm] at (0,0) [label=below:{\phantom{$b+1$}$p_a$\phantom{$b+1$}}] {};

\node [draw,fill,inner sep=0cm,minimum height=0.1cm] at (3.5,0) [label=below:{\phantom{$b+1$}$p_b$\phantom{$b+1$}},label=above:{$p_{i_k}$}] {};
\node [draw,fill,inner sep=0cm,minimum height=0.1cm] at (4.5,0) [label=below:{\phantom{$b+1$}$p_{b+1}$\phantom{$b+1$}}] {};
\node [draw,fill,inner sep=0cm,minimum height=0.1cm] at (8,0) [label=below:{\phantom{$b+1$}$p_d$\phantom{$b+1$}}] {};

\node [draw=gray,fill=gray,inner sep=0cm,minimum height=0.1cm] at (pc) [label=below:{\textcolor{gray}{\phantom{$b+1$}$p_c$\phantom{$b+1$}}}] {};
\node [draw=gray,fill=gray,inner sep=0cm,minimum height=0.1cm] at (pcs) [label=below:{\textcolor{gray}{\phantom{$b+1$}$p_{c'}$\phantom{$b+1$}}}] {};

\draw (-0.5,0) -- (10,0);
\end{tikzpicture}
\end{center}

\begin{center}
\begin{tikzpicture}
\useasboundingbox (-0.5,-1) rectangle (8.5,1);
\clip (-0.5,-0.75) rectangle (8.5,0.75);

\coordinate (pc) at (1,0);
\coordinate (pb) at (3.5,0);
\coordinate (pcs) at (6.5,0);

\draw [gray, fill=black!5] (pc) circle (1.15); 
\draw [gray, fill=black!5] (pb) circle (1.1); 
\draw [gray, fill=black!5] (pcs) circle (1.55); 

\foreach \x in {0,0.5,...,8} {
\node [draw=gray,inner sep=0cm,minimum height=0.1cm] at (\x,0) {};
}

\node [draw,fill,inner sep=0cm,minimum height=0.1cm] at (0,0) [label=below:{\phantom{$b+1$}$p_a$\phantom{$b+1$}}] {};

\node [draw,fill,inner sep=0cm,minimum height=0.1cm] at (pb) [label=below:{\phantom{$b+1$}$p_b$\phantom{$b+1$}},label=above:{$p_{i_k}$}] {};
\node [draw,fill,inner sep=0cm,minimum height=0.1cm] at (4.5,0) [label=below:{\phantom{$b+1$}$p_{b+1}$\phantom{$b+1$}}] {};
\node [draw,fill,inner sep=0cm,minimum height=0.1cm] at (8,0) [label=below:{\phantom{$b+1$}$p_d$\phantom{$b+1$}}] {};

\node [draw=gray,fill=gray,inner sep=0cm,minimum height=0.1cm] at (pc) [label=below:{\textcolor{gray}{\phantom{$b+1$}$p_c$\phantom{$b+1$}}}] {};
\node [draw=gray,fill=gray,inner sep=0cm,minimum height=0.1cm] at (pcs) [label=below:{\textcolor{gray}{\phantom{$b+1$}$p_{c'}$\phantom{$b+1$}}}] {};


\draw (-0.5,0) -- (10,0);
\end{tikzpicture}
\end{center}
\caption{Idealized schematic of the optimal redivision step in the case of $i_k=b$.\label{fig:redivision}}
\end{figure}

==> mergeandreduceframework.tex <==
\subsection{Merge and reduce framework}

Informally, the merge-and-reduce framework can be described as follows. Given is a method to compute a summary/coreset/sublinear data structure for input data. The input stream is read in blocks, and the given method is applied to a block when it has been read; we call the result $B$.

The algorithm maintains a dynamic array and wants to store $B$ in this array. For that purpose, it searches for the first empty spot in $A$. Along the way, the data that is stored in $A$ is merged with (the growing content of) $B$ and subsequently reduced by calling the given method. 

\algorithmus{\texttt{merge-and-reduce-general}}{
\begin{enumerate}
    \item Initialize an empty dynamic array $A$
    \item Read a block of input data and compute a summary/sublinear data structure $B$
    \item Set $i=0$
    \item {\bf While} $A[i]$ is non-empty
    \item \hspace*{0.5cm} Combine the information in $A[i]$ with the information in $B$
    \item \hspace*{0.5cm} Compute a summary/sublinear data structure of the union and store it in $B$ 
    \item \hspace*{0.5cm} Set $i=i+1$
    \item Store $B$ in $A[i]$
\end{enumerate}
}

The important property of the computation tree of merge-and-reduce is that for all $i \ge 0$, the information stored in $A[i]$ (if $A[i]$ is non-empty) represents $2^i b$ input points (where $b$ is the block size), and it is the result of at most $i$ reduction steps. This means that if $n$ input points were read from the stream, then the largest index $i^\ast$ of a non-empty spot in $A[i]$ is in $\mathcal{O}(\log n)$, and the content of $A[i^\ast]$ is the result of $i^\ast$ chained coreset computations. Assume that the multiplicative error of one such computation is an $\epsilon$-fraction, i.e., the value that we want to approximate is approximated such that the estimate is at least $(1-\epsilon)$ times the true value and at most $(1+\epsilon)$ times the true value. 
After $i\ast$ chained computations, the bounds have worsened to $(1-\epsilon)^{i^\ast}$ and $(1+\epsilon)^{i^\ast}$. Now the idea is to perform all calls with a smaller $\epsilon$, namely, $\epsilon' = \epsilon / (2 (\log n +1))$, \todo{notice that this needs knowledge of $n$. this requirement can be removed by more annoyance} such that we get
\[
\left(1+\frac{\epsilon}{2 ( \log n )}\right)^{\log n} \le e^{\epsilon/2} \le \frac{1}{1-\epsilon/2} = 1 + \frac{\epsilon/2}{1-\epsilon/2} \le 1 + \epsilon
\]
and
\[
\left(1-\frac{\epsilon}{2 ( \log n)}\right)^{\log n} \ge (2e)^{-\epsilon/2} \ge e^{-\epsilon} \ge (1-\epsilon).
\]
%Assume that the number of chained coreset computations is $\log (n/s) +1$, i.e., the error is $(1+\epsilon)^{\log (n/s)+1}$.
Notice that the smaller $\epsilon$ usually affects the size of the computed summary/coreset/sublinear data structure.

Three further comments: 

Firstly, setting $\epsilon'$ correctly requires knowledge of $n$. If the length of the stream is unknown, one proceeds like this: Starting with a small estimate $n_0$ on the stream length, one executes the merge-and-reduce framework on the first $n_0$ input points. The result of this is stored away, and the estimate on the stream length is doubled, the next $2 n_0$ items are processed, and so on. In this way, one gets a collection of summaries/coresets/sublinear data structures, one for each guess of the stream lengths. Since the guesses are doubled, the total number is in $\mathcal{O}(\log n)$, so this adds one multiplicative factor of $\log n$ to the asymptotic memory requirement.

Secondly, one single summary/coreset/sublinear data structure can be computed from the stored data (the $\mathcal{O}(\log n)$ entries of $A$, possibly for multiple merge-and-reduce runs with different $n$) by one additional merge and reduce step.

Thirdly, the above description assumes that the used reduction method is deterministic. For randomized constructions, one needs to also adjust the failure probability of each individual call to compensate for the chained computations.


==> twoapproximation.tex <==
\section{A \texorpdfstring{$2$}{2}-approximate curve Simplification Algorithm}\label{appendix:gonzales}

The algorithm in this section resembles the algorithm due to Gonzalez~\cite{G} for $k$-center. Gonzalez' algorithm picks the first center arbitrarily, and then subsequently chooses a point as the next center which is at maximum distance of all previously chosen centers. 

We do something similar: We start with the first vertex of $X$ as the first point of the simplification. In the following iterations, we would like to pick a point that is furthest away from its \lq center\rq, i.e., that attains the current maximum distance between a vertex on $X_k$ and a vertex on $X$ (i.e., in a traversal which we also keep, the distance of this vertex to the point on $X_k$ its mapped to is $\df(X,X_k)$.

However, the order constraint causes complications. Consider a $1$-dimensional curve $X$ in $\mathbb{R}$ with $p_1=0$, $p_2=1$, $p_3=-1$, $p_4=1$, $p_5=-1$, $\ldots$, $p_{n-1}=1$, $p_n=-1$,  (for odd $n$), i.e., a curve that starts at $0$ and then oscillates between $1$ and $-1$. The first simplification $X_1=p_1$ has a Fr\'echet distance of $1$ to $X$. Now every other vertex attains the maximum distance to $p_1$. And in fact, if we choose any vertex except $p_n$, we actually \emph{increase} the Fr\'echet distance. 

Say for example that we choose $p_{n-1}$. Then since we have to traverse $p_{n-1}$ at some point, we have to assign a suffix of $X$ to $p_{n-1}$, in particular, we have to assign $p_n$ to it, implying that $\df(X_2,X)=2$ while $\df(X_1,X)=1$. Notice that this is not a tie-breaking issue: We could move $p_{n-1}$ slightly to $1.1$ to make it the point that is the sole candidate at maximum distance, and the effect would still take place. 
To avoid this problem, we choose a vertex that is at the border of a cluster (i.e., on of its neighbors belongs to a different cluster/interval). This ensures that we can always insert the new vertex on $X_k$ into the current traversal without causing harm. Its cluster will consist of at least itself, and possibly additional points to the left and right.

At first, the change of the algorithm sounds like we lose the most important property of Gonzalez' algorithm since we do no longer choose a point at maximum distance. However, we will pick a border vertex which satisfies that between itself and its center, there is a vertex that currently attains maximum distance. We show that this is sufficient to prove that the algorithms computes a $2$-approximate curve simplification.

%The details of the algorithm an the proof are a bit technical and we defer them to Appendix~\ref{appendix:gonzales}.

\begin{restatable}{theorem}{twoapproxthm}\label{thm:twoapprox}
For any curve $X=p_1,\ldots,p_n$ and and $k \in \mathbb{N}^{\ge 1}$, the simplification $X(I_k)$ computed by algorithm \texttt{approximate-curve-simplification($X,k$)} (see page~\pageref{appendix:gonzales}) is a $2$-approximate curve simplification.
\end{restatable}

Our algorithm constructs a simplification iteratively. After $k$ iterations of our main loop, the computed curve $X_k$ is an approximate curve simplification with $k$ points. The vertices of $X_k$ are always a subset of the vertices of $X$.

In addition to the choice of vertices, the algorithm also maintains a traversal of the two curves $X$ and $X_k$ which gives us an upper bound on their Fr\'echet distance. We do not store this traversal explicitly, but instead store a partitioning of $\{1,\ldots,n\}$ into $k$ intervals. The traversal is implicitly given: While traversing the first interval on $X$, we stay at the first vertex on $X_k$, then we jump from the last point in the interval to the first point on the second interval while jumping to the second vertex on $X_k$, and so on.
We call the vertex on $X_k$ that the traversal stays at while traversing an interval the \emph{center} of that interval.

For convenience, we store the intervals together with their center. 
An interval partitioning $I$ thus is a set of tuples $([a,b],c), a,b,c \in [n]$ such that for all $i \in [n]$, there is exactly one $([a,b],c) \in I$ with $a\le i \le b$.
%We subsequently partition the curve $X=x_1,\ldots,x_n$ into intervals. At any point, $I$ contains a collection of disjoint intervals that cover $\{1,\ldots,n\}$, together with the index of the point that the points in the interval are mapped to. For example, we start by adding the interval $[1,n],1$, which means that $X_1$ consists of $x_1$ and all points on $X$ are mapped to $x_1$.
We iteratively compute these interval partitionings, $I_k$ is the partitioning into $k$ intervals.
For example, the first simplification that we compute is $X_1 = p_1$, and the corresponding traversal is implicitly given by $I_1=\{([1,n], 1)\}$, i.e., a partitioning into a single interval which shall be traversed while staying at $p_1$ on $X_k$.

We define the \emph{radius} of any $([a,b],c)\in I$ as
\[
r(a,b,c) := \max\{d(p_i,p_j)\mid a \le j \le b\}.
\]
For convenience, we set $r(a,b,c)=0$ if $a > b$.
Notice that for the traversal $T$ implicitly defined by the interval partitioning $I$, we have 
\[
\max_{(i_u,j_u)\in T} d(p_{i_u},q_{j_u}) = \max_{([a,b],c)\in I} r(a,b,c).
\]
Thus, $\max_{([a,b],c)\in I_k} r(a,b,c)$ is an upper bound on the Fr\'echet distance between $X$ and $X_k$ at any point in time.

For an interval partitioning $I$, we say that the \emph{cutoff vertices} are all vertices that lie at the end of an interval, and we refer to the set of indices of cutoff vertices as \emph{cutoff indices}, i.e., the set of cutoff indices is
\[
C(I) := \bigcup\limits_{([a,b],c)\in I}  \{a,b\}
\]
The set of center indices is $Z(I) := \{ c \mid \exists a,b \in [n]: ([a,b],c)\in I\}$. We say that a cutoff vertex $p_i, i\in C(I)$ is \emph{free} if $i\notin Z(I)$, and \emph{taken} otherwise. We get the simplification $X(I)$ by concatenating the vertices $p_c, c \in Z(I)$ in increasing order of their indices.

Our algorithm subsequently chooses a cutoff vertex as the next vertex to be added to $X_k$, and the vertex that is chosen is one that is at maximum distance from the center of its interval. The second vertex thus is $p_n$, since this is the only free cutoff vertex for the interval partitioning $\{([1,n],1)\}$. 
The only thing to be computed for the second simplification is how to split the interval $[1,n]$, we do this optimally by computing the vertex $i \in [1,n]$ which minimizes
\[
split(1,n,i) = 
\max\{ r(1,i,1), r(i+1,n,n)\}.
\]

For the subsequent iterations, we always pick a cutoff point $p_k$ to be added to $X_k$ by choosing it from an interval in $I_{k-1}$ of maximum radius. Then we optimally redivide two intervals in order to incorporate the new vertex. Before describing this in more detail, we give a pseudo-code description of the algorithm's main routine: 

\algorithmus{\texttt{approximate-curve-simplification({\normalfont a curve} $X=p_1,\ldots,p_n$, $k_{\max} \in\mathbb{N}^{\ge 1}$)}}{
\begin{enumerate}
  \setlength{\itemsep}{0.0cm}
  \item Set $I_1=\{([1,n],1)\}$
  \item Compute $b=\arg\min\{split(1,n,i)\mid 1\le i \le n\} $
  \item Set $I_2=\{([1,b],1),([b+1,n],n)\}$
  \item {\bf For} $k=3$ {\bf to} $k_{max}$ {\bf do}
    \item \hspace*{0.5cm} Choose an $([a,b],c)\in I_{k-1}$ which maximizes $r(a,b,c)$. 
  \item \hspace*{0.5cm} {\bf If} $r(a,b,c) =0$, {\bf Return} $X(I_{k-1})$
  \item \hspace*{0.5cm} {\bf If} $p_a$ is taken, {\bf then} set $i_k=b$, {\bf else} if $p_b$ is taken, {\bf then} set $i_k=a$
  \item \hspace*{1cm} {\bf Else} (in this case, $p_a$ and $p_b$ are both free) 
  \item \hspace*{1.5cm} {\bf} If $r(a,c,c) > r(c,b,c)$ {\bf then} set $i_k=a$ {\bf else} set $i_k=b$
  %\item \hspace*{0.5cm} Set $i_k=a$ or $i_k=b$ such that $p_i$ is free
  %(either $p_a$ or $p_b$ will always be free)
  \item \hspace*{0.5cm} Compute $I_k=$\texttt{optimal-redivision}$(I_{k-1},[a,b], i_k)$
  \item {\bf Return} $X(I_{k_{\max}})$
  %\item \hspace*{0.5cm} Let $([a,b],c)\in I$ be the interval that $x_i$ lies in, i.e., $i=a$ or $i=b$ 
  %\item Compute $\ell = \arg\max\{ \max\{ d(x_a,x_{\ell}, d(x_{\ell},x_b) \} \mid [a,b],\ell)\in I \}$
  %\item Compute $a' = \arg\min\{leash(a,\ell,i)\mid a \le i \le \ell$ and $b' = \arg\min\{leash(\ell,b,i)\mid \ell \le i \le b\}$
  %\item Replace $([a,b],\ell)$ in $I$ by $([a,a'-1],?)$
%	\item \hspace*{0.5cm} Find a point $x_i$, $i\in[n]$, with $d(x_i,\mu(x_i))=\df(X,X_k)$ 
  %\item \hspace*{0.5cm} Set $I_i = I_{i-1} \cup \{i\}$
\end{enumerate}
}

Observe that the above algorithm is well-defined in the sense that in Step 7/8, either $p_a$ or $p_b$ is always free. That is because we only get to this point if the chosen interval has a strictly positive radius. 
\begin{observation}
Any interval $([a,b],c)\in I_{k-1}$ with $r(a,b,c) > 0$ contains a free cutoff vertex.
\end{observation}
\begin{proof}
An interval with strictly positive radius contains at least two vertices and thus at least two cutoff vertices, out of which at most one can be the center. The remaining one is free.
\end{proof}

\input{fig-redivision}
For the optimal redivision, we have to solve the following task (also see Figure~\ref{fig:redivision}, where the notation follows below pseudo code).
Considering the interval that $i_k$ lies in, we create a new interval that consists at least of $i_k$, but is extended optimally to include parts from the interval $i_k$ lies in and the neighboring interval. Notice that the $i_k$ that we pick always lies in an interval that has a neighbor on the side of $i_k$, since $i_k$ is a cutoff point and lies between two intervals per definition. For finding the optimal way to split the two involved intervals, we use a generalization of the above split definition:
\[
split(a,b,c_1,c_2,i) =\max\{ r(a,i,c_1), r(i+1,b,c_2)\}.
\]
Given an interval $[a,b]$ and two possible centers $c$ and $d$, $split(a,b,c,d,i)$ is the maximum radius that is incurred from splitting $[a,b]$ at $i$ and assigning the left part to $c$ and the right part to $d$.
%Assign at least the point to itself, plus an optimally chosen amount of the left and right neighbor interval. 
Given this definition, the following function replaces $[a,b]$ and the neighboring interval and replaces them by three intervals covering the same ground set, where the middle interval contains $i_k$ and possibly additional indices.

\algorithmus{\texttt{optimal-redivision}(I,[a,b],k)}{
\begin{enumerate}
    \item Let $c\in [n]$ be the index with $([a,b],c)\in I$
    \item {\bf If} $i_k=b$ {\bf then}
    \item \hspace*{0.5cm} Let $d\in [n]$ be such that $([b+1,d],c')\in I$ for some $c' \in [n]$ 
    \item \hspace*{0.5cm} Set $a' = \arg\min_{a \le i \le b-1} split(a,b-1,c,i_k,i)$, $b'= \arg\min_{b \le i \le d} split(b,d,i_k,c',i)$
    %\item \hspace*{0.5cm} Compute $a' = \arg\min_{a\le i \le b}\{ \max\{r(a,i,c),r(i+1,b,k)\} \mid a \le a' \le b\}$ 
        %and 
    %\item \hspace*{0.5cm} Compute $b' = \arg\min\{\max\{r(b+1,j,k),r(j+1,b'+1,c')\} \mid b+1 \le b' \le d\}$
    \item \hspace*{0.5cm} Replace $([a,b],k)$ and $([b+1,d],c')$ in $I$ by $([a,a'],c)$, $([a'+1,b'],k)$ and $([b'+1,b],c)$
    \item {\bf Else}
    \item \hspace*{0.5cm} Let $d\in [n]$ be such that $([d,a-1],c')\in I$ for some $c' \in [n]$ 
    \item \hspace*{0.5cm} Set $a'=\arg\min_{d \le i \le a-1} split(d,a-1,c',i_k,i)$, $b'=\arg\min_{a \le i \le b} split(a,b,i_k,c,i)$
    %\item \hspace*{0.5cm} Compute $a' = \arg\min\{ \max\{r(d,i,c'),r(i+1,a-1,k)\} \mid d \le a' \le a-1\}$ 
    %\item \hspace*{0.5cm} Compute $b' = \arg\min\{\max\{r(a,j,k),r(j+1,b,c)\} \mid a \le b' \le b\}$
    \item \hspace*{0.5cm} Replace $([d,a-1],c')$ and $([a,b],k)$ in $I$ by $([d,a'],c')$, $([a'+1,b'],k)$ and $([b'+1,b],c)$ 
    \item {\bf Return} $I$
\end{enumerate}
}

\input{fig-algo-example.tex}
Figure~\ref{fig:algoexample} shows a sample execution of the algorithm. 
\begin{observation}\label{obs:mondecr}
The upper bound on $\df(X,X(I_k))$ is monotonically decreasing.
\end{observation}

\twoapproxthm
\begin{proof}
First observe that $X(I_1)$ is a $2$-approximate curve simplification for $k=1$: Assume $O_1=o$ is an optimal curve simplification with one point. Then the only feasible traversal for $X$ and $O_1$ will traverse $X$ while staying at $o$ on $X_k$, i.e., $d(o,p_j)\le \df(X,O_1)$ for all $j \in [n]$. Since by the triangle inequality, $d(p_1,p_j) \le d(p_1,o) + d(o,p_j)\le 2 \df(X,O_1)$ is true for any $j\in [n]$, we see that $X(I_1)$ is a $2$-approximate curve simplification.

In the following, let $O_k=o_1,\ldots,o_k$ be an optimal curve simplification for $X$ with $k$ vertices, and let $T_{\opt}$ be an optimal traversal of $X$ and $O_k$. 
For all $j\in[k]$, let $A(o_j)$ be the set of points on $X$ that are traversed on $X$ while $T_{\opt}$ stays at $o_j$.

The case $k=2$ is a bit special and easier to prove than the general case.
Since $T_{\opt}$ has to start in $p_1$ and to end in $p_n$, we know that $p_1 \in A(o_1)$ and $p_n \in A(o_2)$. For all $p_j \in A(o_1)$, we thus have $d(p_j,p_1)\le 2\cdot\df(X,O_2)$, and for all $p_j \in A(o_2)$, we have $d(p_j,p_n)\le 2\cdot\df(X,O_2)$, both by the triangle inequality. 
We can thus use the traversal that traverses $A(o_1)$ while staying at $p_1$ on $X(I_2)$ and traverses $A(o_2)$ while staying at $p_n$ on $X(I_2)$ to show that $\df(X,X(I_2))\le 2 \cdot \df(X,O_2)$.

Now let $k>2$ be fixed. 
%Let $O_k=o_1,\ldots,o_k$ be an optimal curve simplification for $X$ with $k$ points, and let $T_{\opt}$ be an optimal traversal of $X$ and $O_k$. 
%For all $j\in[k]$, let $X_{o_j}$ be the set of points on $X$ that are traversed on $X$ while $T_{\opt}$ stays at $o_j$.
Here, we consider two cases.
\\
The first case occurs if for all $j\in [k]$, there exists a vertex $p({o_j}) \in A(o_j) \cap Z(I_k)$. In other words, every of the $k$ intervals induced by the optimum solution contains exactly one center from our simplification.
In this case, we can proceed as in the case $k=2$: 
%The first case occurs if for all $j\in [k]$, there exists a point $p({o_j})$ on $X(I_k)$ which lies in $X_{o_j}$. In other words: Every of the $k$ subcurves that are induced by $O_k$ contains at least one point which is part of our approximate simplification $X(I_k)$. Then $\df(X,X(I_k)\le 2\cdot \df(X,O_k)$ is true: 
Construct $T'$ from $T_{\opt}$ by exchanging $o_j$ by the $j$th point on $X_k$. Since $p({o_j}) \in A(o_j)$, its distance to $o_j$ is at most $\df(X,O_k)$, and for all $p_i \in A(o_j)$, $d(p(o_j),p_i)\le 2 \df(X,O_k)$.
Thus, $\df(X,X(I_k))\le 2\cdot \df(X,O_k)$. 

The second case occurs if there is an interval which does not contain a point from $Z(I_k)$. This implies that there also is an interval which contains two points from $Z(I_k)$. We use this information to show that $X(I_{k-1})$ was already a good simplification even compared to $O_k$.

Let $p_x, p_y \in Z(I_k)$ be chosen such that $p_x, p_y \in A({o_j})$ for some $j\in [k]$, and choose the naming such that $y$ was added to $X(I)$ in an earlier iteration than $x$, and let $k'$ be the iteration in which $p_y$ was added to $I$ (i.e., $p_y$ was actually added to $X(I_{k'-1})$ to form $X(I_{k'})$). It is possible that $k'=k$, but that is not necessary. 
Furthermore, we choose $x$ and $y$ such that between $p_x$ and $p_y$, no point on $X$ is in $Z(I_{k})$.
Without loss of generality, we assume that $x < y$ (the index of $p_x$ is smaller than the index of $p_y$). 

We even show that $X(I_{k'-1})$ is a good simplification compared to $O_k$, more precisely, that the implicitly stored traversal has at most twice the cost as an optimal solution. By Observation~\ref{obs:mondecr}, that implies that $X(I_k)$ is a $2$-approximate curve simplification as well.

To do so, we again distinguish two cases depending on the interval $([a,b],z) \in I_{k'-1}$ that contains $p_y$, i.e. the interval with $a \le y \le b$. 
We know that no vertex between $p_x$ and $p_y$ is in $Z(I_k)$, and thus $Z(I_{k'-1})$ also contains no vertex between $p_x$ and $p_y$. The vertex $p_y$ itself is not in $Z(I_{k'-1})$, it was a cutoff point in iteration $k'$. What we do not know is whether $p_x$ is in $[a,b]$ or whether $x < a$. 

If $a \le x \le b$, then $p_x$ was the center of $[a,b]$, i.e., $z=x$ (it was added to the centers before $p_y$, so it is already a center, and there is exactly one center in $[a,b]$). By our choice of the next center $p_y$ as a cutoff point in an interval of maximum radius, we know  $r(a,b,x)=\df(X,X(I_{k'}-1))$. Furthermore, $r(x,y,x) = r(a,b,x)$ has to be true: Either $p_y$ was the only free cutoff vertex in $[a,b]$, then $p_x$ has to be the other cutoff vertex, i.e., $a=x$ and $b=y$, or both cutoff vertices were free, but then we chose the cutoff vertex for which the largest distance to $p_x$ is maximal, also implying that $r(x,y,x)=r(a,b,x)$. 
Now this does not mean that the distance between $p_x$ and $p_y$ is necessarily large, however, it means that there is a point $p_i$ with $x \le i \le y$ such that $d(p_x,p_i) = r(x,y,y) = r(a,b,x) = \df(X,X(I_{k'-1}))$. And since $p_x, p_y \in A(o_j)$, monotonicity guarantees that $p_i \in A(o_j)$ as well. And this means that the maximum distance from any point in $A(o_j)$ to $o_j$ is at least $\df(X,X(I_{k'-1})) / 2$, i.e., $\df(X,X(I_{k'-1})) \le 2 \df(X,O_k)$.

Some additional argumentation is required when $x < a$, or, in other words, $p_x$ is in a different interval in $I_{k'-1}$ than $p_y$. Since $p_y$ is a cutoff point, it is thus the first point of its interval, i.e., $a=y$, and the interval containing $p_y$ ends at $y-1$ and has $p_x$ as its center (the center of $[a,b]$ is $p_z$). 
Let $[a',y-1,x]\in I_{k'-1}$ be the interval with $a' \le x \le y-1$. 
So we have an interval $[a',y-1]$ with center $p_x$, and an interval $[y,b]$ with center $p_z$, and $p_y$ is a cutoff point between the two intervals. Now we need that the cutoff position was chosen optimally at some point in the algorithm (we either had $p_x$ or $p_z$ first, and then computed an optimal split). Indeed, we know that $\max\{r(x,i,x),r(i+1,z,z)\}$ is minimized by setting $i=y-1$. If we choose to split at $y$, then the maximum radius can only increase, and not decrease. Since $r(y+2,z,z) \le r(y+1,z,z)$, this means that $r(x,y,x) \ge \max\{r(x,i,x),r(i+1,z,z)\}$. Furthermore, similarly to the first subcase, we know that $p_y$ was chosen in a way that ensures that $r(y+1,z,z) = r(a,b,z) = \df(X,X(I_{k'-1})$. We have thus arrived at a similar point in the argumentation as in the first subcase: We know that $r(x,y,x) \ge \df(X,X(I_{k'-1})$. Since $p_x, p_y \in A(O_j)$, and so are all $p_i$ with $x \le i \le y$, this implies that $\df(X,O_k) \ge \df(X,X(I_{k'-1}))/2$.

That completes the proof.
\end{proof}
